Understanding Influence Maximization via Higher-Order Decomposition

Given its vast application on online social networks, Influence Maximization (IM) has garnered considerable attention over the last couple of decades. Due to the intricacy of IM, most current research concentrates on estimating the first-order contribution of the nodes to select a seed set, disregarding the higher-order interplay between different seeds. Consequently, the actual influence spread frequently deviates from expectations, and it remains unclear how the seed set quantitatively contributes to this deviation. To address this deficiency, this work dissects the influence exerted on individual seeds and their higher-order interactions utilizing the Sobol index, a variance-based sensitivity analysis. To adapt to IM contexts, seed selection is phrased as binary variables and split into distributions of varying orders. Based on our analysis with various Sobol indices, an IM algorithm dubbed SIM is proposed to improve the performance of current IM algorithms by over-selecting nodes followed by strategic pruning. A case study is carried out to demonstrate that the explanation of the impact effect can dependably identify the key higher-order interactions among seeds. SIM is empirically proved to be superior in effectiveness and competitive in efficiency by experiments on synthetic and real-world graphs.

==> SDM '23 Sobol Influence Maximization/draft.tex <==
\subsection{Old Intro}
Current IM methods are typically divided into simulation-based and proxy-based categories ~\cite{li2018influence}. Unfortunately, neither of them is able to offer consistently trustworthy solutions in a timely manner. Specifically, this deficiency stems primarily from:
\textbf{(1) Relying on the first-order properties.}
For the sake of efficiency, some proxy-based IM algorithms simply sum the impacts of every seed, while other approaches update the proxies lightly between two successive greedy stages by deleting the selected seed from the network~\cite{chen2009efficient, yan2019minimizing, zhang2022blocking}. 
% The majority of simulation-based algorithms likewise follow a greedy technique that only examines the contribution of the first order. 
Both approaches emphasize the first-order contribution, while disregarding the interaction efficacy among the seeds. 
However, because of the combinatorial impact in the seed set, the actual influence spread is heavily influenced by this interaction~\cite{kempe2003maximizing, chen2009efficient, li2018influence}.
Figure~\ref{fig:1} illustrates an example of this interaction by depicting the influence distribution of a four-node seed set. Three of them (nodes 1, 2, and 3) are close to one another, whereas the fourth is far away. During $t$ stages of the propagation, the influence flows propagated from the first three seeds may overlap (gray areas), cancelling a portion of their overall influence spread and failing to maximize their joint coverage.
\textbf{(2) The imbalance of effectiveness and efficiency}.
As one main type of IM algorithms, the simulation-based methods are theoretically guaranteed to have a high approximation performance but lack scalability ~\cite{arora2017debunking}. By greedily adding the node with the highest marginal spread in each step, this thread of methods is proved to guarantee a $(1 - \frac{1}{e})$ approximation ratio~\cite{kempe2003maximizing}. However, multiple rounds of simulations are required to evaluate the marginal spread for each candidate nodes in each round, making the heuristic extremely slow when the graph size is large. 
% Research following this thread made tremendous effort on reducing the complexity yet still fails to accelerate these methods enough. 
As another important category of IM approaches, the proxy-based algorithms are applicable to large social networks, but there is no assurance that a good approximation ratio can be reached~\cite{li2018influence}. In IM community, most research still focus on searching for faster but less accurate simulation methods~\cite{cheng2013staticgreedy, borgs2014maximizing} or designing better proxies that usually come with higher computational loads~\cite{yan2019minimizing, zhang2022blocking}.

\textcolor{red}{[todo]}
Besides, current IM researches typically focus on how to identify a set of seeds that maximize the expected influence spread. Other than that, which seed or seeds account for the greatest contribution to the final influence has not been discussed. Although some of the heuristics select seeds according to transparent measures such as centrality metrics, the process through which the seed set results in the final influence spread is still hidden. Nonetheless, due to the high stake of the quality of the solution, this explanation towards the selected seed set is necessary. 

In this work, we will employ approaches that can disentangle and quantitatively evaluate higher-order interactions among selected seeds.
%\textcolor{red}{rearrange order}
\textcolor{red}{[todo]}Existing work has various drawbacks:
\textbf{Local interpretation methods}, including LIME~\cite{ribeiro2016should} and Grad-cam~\cite{selvaraju2017grad}, focus only on local neighborhoods and disregard the global impact of the seeds and their higher-order interactions.
\textbf{Marginal contribution}~\cite{catav2021marginal} does not separate the higher-order interaction effects from the main effect thus fails to quantify the interactions among seeds.
\textbf{The Shapley value}~\cite{roth1988shapley} distributes the higher-order interaction among the seeds and tends to overestimate the contribution of the nodes with larger influence overlaps with others.
Beyond that, none of them well handle higher-order interactions in the IM scenario.
Comparatively, the Sobol indices can overcome the shortcomings of the above alternatives. 
\textbf{(1)} It is a global sensitivity method that considers a seed's global impact within the seed set. 
\textbf{(2)} The first-order effect and the higher-order interactions can be separated with a clear cut utilizing the corresponding Sobol indices. 
\textbf{(3)} The Sobol index that describes the total effect of a seed includes the whole contribution brought by the higher-order interactions between the seed and any subset of rest of the seed set, thus precisely captures the influence loss if the seed is not selected.
Therefore, we select the Sobol indices as an effective method for decomposing a seed set's influence spread.

To address these issues, this paper introduces a global sensitivity analysis methods, namely the Sobol indices~\cite{sobol1993sensitivity, wagener2019has}, into the explanation of the seed set selected by IM algorithms. 
In particular, the global contribution of a seed node is measured using the Sobol total index, which reflects its overall contribution to the influence spread. 
The contribution composition is then explained using first- and higher-order Sobol indices. Importantly, the interactions between seed nodes are identified quantitatively with a higher-order index, which explains why most first-order approaches fail to appropriately identify the contributions of nodes.
% In IM problems, the separate contribtution of each node within the seed set can be estimated by its Sobol total index, while the interactions among the nodes are evaluated by the higher-order Sobol indices. 
%Figure~\ref{fig:1} demonstrates the connection between the IM problem and the Sobol indices. The left of the figure shows the influence of a seed set of four nodes. Among them, three nodes (node 1,2,3) are close to each other while the last one (node 4) is far away. During the $t$ steps of the propagation, the influence flows coming out of the seeds may meet each other, creating an influence overlap that diminishes the total influence. While conducting the sensitive analysis with the Sobol indices, the contribution of each node and the influence overlaps among the nodes can be quantified as shown on the right side of the figure.
% \textcolor{red}{explain more details, each notation in fig need explanation, such as node 1 xxx, node 2 xxx, so xxx}. 
%After obtaining the indices, the seeds can be ranked accordingly. This ranking method can be utilized to select the seed to be removed when the budget constraint shrinks
%, or facilitate the selection of the seed set at the first place.
%. According to this explanatory method, an IM algorithm utilized the higher-order interactions named~\algo~is proposed to increase the quality of the solution.

% Contributions
This paper's primary contributions include:
\begin{itemize}

\item \textbf{Explain the influence spread and evaluate the seed set}: 
%Our approach is independent to the IM methods through which the seed set is selected. 
Given any seed set and the corresponding graph,
%generated by any IM method solving an IM problem on any diffusion model
each seed's contribution to the influence spread can be measured with the proposed explanatory method regardless of the IM algorithm that generates the seed set. Thus, this method can serve as a universal post-hoc explanation of an IM algorithm.

\item \textbf{Propose a higher-order analysis}:
To the best of our knowledge, this paper serves as the first discussion on the quantification of the influence overlap among the seeds. This new method suggests a new direction for IM research.

\item \textbf{Provide a new IM schema}:
We propose a light-weighted method named~\algo. By introducing the global sensitivity analysis,~\algo~overcomes the scalability and dependability issues in the literature and provides a new schema for designing IM methods. 
Empirical experiments on real-world and synthetic datasets demonstrate that~\algo~achieves superior performance in a reasonable amount of time.

%By selecting seed candidates over the budget constraint and removing the least important candidate iteratively until the constraint is met,~\algo~achieves superior performance with an acceptable time complexity.
%\item \textbf{Conduct extensive experiments on synthetic and real-world networks}: 
%The effectiveness of our explanation method is evaluated on both synthetic dataset and real-world data. Results show that the evaluations provided by this framework are robust across different networks.~\algo~is compared with multiple baselines and achieves a superior performance.
\end{itemize}

% \colorbox{yellow}{1st paragraph: Intro to general IM; interpretability and higher-order interaction}

% \textcolor{red}{application background} influence maximization is widely applied in xxx

% \colorbox{yellow}{2nd paragraph: Show an example why higher-order can explain, and previous methods are doing something they do not plan w/ Fig!}

% \colorbox{yellow}{Fig: 3/4 dots. 4 circles like in experiment, biggest one has interaction with other two, while the last one far away.}

==> draft.tex <==
\subsection{Old Intro}
Current IM methods are typically divided into simulation-based and proxy-based categories ~\cite{li2018influence}. Unfortunately, neither of them is able to offer consistently trustworthy solutions in a timely manner. Specifically, this deficiency stems primarily from:
\textbf{(1) Relying on the first-order properties.}
For the sake of efficiency, some proxy-based IM algorithms simply sum the impacts of every seed, while other approaches update the proxies lightly between two successive greedy stages by deleting the selected seed from the network~\cite{chen2009efficient, yan2019minimizing, zhang2022blocking}. 
% The majority of simulation-based algorithms likewise follow a greedy technique that only examines the contribution of the first order. 
Both approaches emphasize the first-order contribution, while disregarding the interaction efficacy among the seeds. 
However, because of the combinatorial impact in the seed set, the actual influence spread is heavily influenced by this interaction~\cite{kempe2003maximizing, chen2009efficient, li2018influence}.
Figure~\ref{fig:1} illustrates an example of this interaction by depicting the influence distribution of a four-node seed set. Three of them (nodes 1, 2, and 3) are close to one another, whereas the fourth is far away. During $t$ stages of the propagation, the influence flows propagated from the first three seeds may overlap (gray areas), cancelling a portion of their overall influence spread and failing to maximize their joint coverage.
\textbf{(2) The imbalance of effectiveness and efficiency}.
As one main type of IM algorithms, the simulation-based methods are theoretically guaranteed to have a high approximation performance but lack scalability ~\cite{arora2017debunking}. By greedily adding the node with the highest marginal spread in each step, this thread of methods is proved to guarantee a $(1 - \frac{1}{e})$ approximation ratio~\cite{kempe2003maximizing}. However, multiple rounds of simulations are required to evaluate the marginal spread for each candidate nodes in each round, making the heuristic extremely slow when the graph size is large. 
% Research following this thread made tremendous effort on reducing the complexity yet still fails to accelerate these methods enough. 
As another important category of IM approaches, the proxy-based algorithms are applicable to large social networks, but there is no assurance that a good approximation ratio can be reached~\cite{li2018influence}. In IM community, most research still focus on searching for faster but less accurate simulation methods~\cite{cheng2013staticgreedy, borgs2014maximizing} or designing better proxies that usually come with higher computational loads~\cite{yan2019minimizing, zhang2022blocking}.

\textcolor{red}{[todo]}
Besides, current IM researches typically focus on how to identify a set of seeds that maximize the expected influence spread. Other than that, which seed or seeds account for the greatest contribution to the final influence has not been discussed. Although some of the heuristics select seeds according to transparent measures such as centrality metrics, the process through which the seed set results in the final influence spread is still hidden. Nonetheless, due to the high stake of the quality of the solution, this explanation towards the selected seed set is necessary. 

In this work, we will employ approaches that can disentangle and quantitatively evaluate higher-order interactions among selected seeds.
%\textcolor{red}{rearrange order}
\textcolor{red}{[todo]}Existing work has various drawbacks:
\textbf{Local interpretation methods}, including LIME~\cite{ribeiro2016should} and Grad-cam~\cite{selvaraju2017grad}, focus only on local neighborhoods and disregard the global impact of the seeds and their higher-order interactions.
\textbf{Marginal contribution}~\cite{catav2021marginal} does not separate the higher-order interaction effects from the main effect thus fails to quantify the interactions among seeds.
\textbf{The Shapley value}~\cite{roth1988shapley} distributes the higher-order interaction among the seeds and tends to overestimate the contribution of the nodes with larger influence overlaps with others.
Beyond that, none of them well handle higher-order interactions in the IM scenario.
Comparatively, the Sobol indices can overcome the shortcomings of the above alternatives. 
\textbf{(1)} It is a global sensitivity method that considers a seed's global impact within the seed set. 
\textbf{(2)} The first-order effect and the higher-order interactions can be separated with a clear cut utilizing the corresponding Sobol indices. 
\textbf{(3)} The Sobol index that describes the total effect of a seed includes the whole contribution brought by the higher-order interactions between the seed and any subset of rest of the seed set, thus precisely captures the influence loss if the seed is not selected.
Therefore, we select the Sobol indices as an effective method for decomposing a seed set's influence spread.

To address these issues, this paper introduces a global sensitivity analysis methods, namely the Sobol indices~\cite{sobol1993sensitivity, wagener2019has}, into the explanation of the seed set selected by IM algorithms. 
In particular, the global contribution of a seed node is measured using the Sobol total index, which reflects its overall contribution to the influence spread. 
The contribution composition is then explained using first- and higher-order Sobol indices. Importantly, the interactions between seed nodes are identified quantitatively with a higher-order index, which explains why most first-order approaches fail to appropriately identify the contributions of nodes.
% In IM problems, the separate contribtution of each node within the seed set can be estimated by its Sobol total index, while the interactions among the nodes are evaluated by the higher-order Sobol indices. 
%Figure~\ref{fig:1} demonstrates the connection between the IM problem and the Sobol indices. The left of the figure shows the influence of a seed set of four nodes. Among them, three nodes (node 1,2,3) are close to each other while the last one (node 4) is far away. During the $t$ steps of the propagation, the influence flows coming out of the seeds may meet each other, creating an influence overlap that diminishes the total influence. While conducting the sensitive analysis with the Sobol indices, the contribution of each node and the influence overlaps among the nodes can be quantified as shown on the right side of the figure.
% \textcolor{red}{explain more details, each notation in fig need explanation, such as node 1 xxx, node 2 xxx, so xxx}. 
%After obtaining the indices, the seeds can be ranked accordingly. This ranking method can be utilized to select the seed to be removed when the budget constraint shrinks
%, or facilitate the selection of the seed set at the first place.
%. According to this explanatory method, an IM algorithm utilized the higher-order interactions named~\algo~is proposed to increase the quality of the solution.

% Contributions
This paper's primary contributions include:
\begin{itemize}

\item \textbf{Explain the influence spread and evaluate the seed set}: 
%Our approach is independent to the IM methods through which the seed set is selected. 
Given any seed set and the corresponding graph,
%generated by any IM method solving an IM problem on any diffusion model
each seed's contribution to the influence spread can be measured with the proposed explanatory method regardless of the IM algorithm that generates the seed set. Thus, this method can serve as a universal post-hoc explanation of an IM algorithm.

\item \textbf{Propose a higher-order analysis}:
To the best of our knowledge, this paper serves as the first discussion on the quantification of the influence overlap among the seeds. This new method suggests a new direction for IM research.

\item \textbf{Provide a new IM schema}:
We propose a light-weighted method named~\algo. By introducing the global sensitivity analysis,~\algo~overcomes the scalability and dependability issues in the literature and provides a new schema for designing IM methods. 
Empirical experiments on real-world and synthetic datasets demonstrate that~\algo~achieves superior performance in a reasonable amount of time.

%By selecting seed candidates over the budget constraint and removing the least important candidate iteratively until the constraint is met,~\algo~achieves superior performance with an acceptable time complexity.
%\item \textbf{Conduct extensive experiments on synthetic and real-world networks}: 
%The effectiveness of our explanation method is evaluated on both synthetic dataset and real-world data. Results show that the evaluations provided by this framework are robust across different networks.~\algo~is compared with multiple baselines and achieves a superior performance.
\end{itemize}

% \colorbox{yellow}{1st paragraph: Intro to general IM; interpretability and higher-order interaction}

% \textcolor{red}{application background} influence maximization is widely applied in xxx

% \colorbox{yellow}{2nd paragraph: Show an example why higher-order can explain, and previous methods are doing something they do not plan w/ Fig!}

% \colorbox{yellow}{Fig: 3/4 dots. 4 circles like in experiment, biggest one has interaction with other two, while the last one far away.}
